Simulation and Real-World Evaluation of Attack Detection Schemes

A variety of anomaly detection schemes have been proposed to detect malicious attacks to Cyber-Physical Systems. Among these schemes, Dynamic Watermarking methods have been proven highly effective at detecting a wide range of attacks. Unfortunately, in contrast to other anomaly detectors, no method has been presented to design a Dynamic Watermarking detector to achieve a user-specified false alarm rate, or subsequently evaluate the capabilities of an attacker under such a selection. This paper describes methods to measure the capability of an attacker, to numerically approximate this metric, and to design a Dynamic Watermarking detector that can achieve a user-specified rate of false alarms. The performance of the Dynamic Watermarking detector is compared to three classical anomaly detectors in simulation and on a real-world platform. These experiments illustrate that the attack capability under the Dynamic Watermarking detector is comparable to those of classic anomaly detectors. Importantly, these experiments also make clear that the Dynamic Watermarking detector is consistently able to detect attacks that the other class of detectors are unable to identify.

==> Experimental.tex <==
\section{Real World Implementation}
\label{sec:exp}
In this section we draw further comparison between the older algorithms and the newer Dynamic Watermarking detector, using a segway robot performing path following. Because the real world system explored in this section is not open loop stable, we no longer make use of the notion of the attack capability. Instead we use two sample attacks to demonstrate each detectors capabilities. Furthermore we show that adding a watermark to a dynamic system leads to only marginal reduction in performance, while increasing the detectability of certain attacks. The experimental setup, includes a segway robot with path following control. Localization is provided by google cartographer \cite{Hess2016} using planar lidar, and wheel odometry measurements. For the purpose of control an LTI model was fitted to the observed data yielded the following model:

\begin{figure}[ht]
    \centering
    \includegraphics[trim={0 0 0 0},clip,width=\columnwidth]{figures/slam_spoofing_1.png}
    \caption{Caption}
    \label{fig:error_cord}
\end{figure}

\Ram{Please be kind to your reader and explain what this section will show before going into detail. Also please make sure to reference all figures in the text.}

\begin{equation}
\label{eq:error}
\begin{bmatrix}
e_{\ell,n+1}\\
e_{s,n+1}\\
e_{\theta,n+1}\\
e_{v,n+1}\\
e_{\dot{\theta},n+1}
\end{bmatrix}
=\begin{bmatrix}
e_{\ell,n}+(0.0478\tilde{v}_n)e_{\theta,n}-(0.045\dot{\tilde{\theta}}_n)e_{s,n}\\
e_{s,n}+(0.0478)e_{v,n}+(0.045\dot{\tilde{\theta}}_n)e_{\ell,n}\\
e_{\theta,n}+0.045e_{\dot{\theta},n}\\
e_{v,n}-0.1e_{v,n-4}+0.1u_{v,n}\\
0.6e_{\dot{\theta},n}+0.15e_{\dot{\theta},n-4}+0.24u_{\dot{\theta},n}
\end{bmatrix}
\end{equation}
where the state is represented in trajectory error coordinates for a given nominal trajectory as shown in figure \ref{fig:error_cord}, $e_{v,n},e_{\dot{\theta},n}$ are the error in the velocity and angular velocity, $\tilde{v}_n,\dot{\tilde{\theta}}_n$ are the nominal velocity and angular velocity and $u_{v,n},u_{\dot{\theta},n}$ are the deviation from the nominal inputs. 

For a constant nominal velocity of $0.6m/s$ and angular velocity of $0 rad/s$ this model can be represented as an LTI model with state vector $x=[e_{\ell,n}~
e_{s,n}~
e_{\theta,n}~
e_{v,n}~
e_{\dot{\theta},n}~
e_{v,n-1}~
e_{v,n-2}~
e_{v,n-3}~
e_{\dot{\theta},n-1}~
e_{\dot{\theta},n-2}~
e_{\dot{\theta},n-3}]^T$. For the sake of brevity the A and B matrices will not be stated explicitly. The feedback gain matrix $K$  was found to make the closed loop system schurr stable and is approximately:
\begin{align}
    K=\begin{bmatrix}
    0 & -1.639 \\ 0 & -1.984 \\ -0.313 & 0\\ -0.212 & 0 \\ 0 & -0.384 \\ 0.019 & 0\\ 0.020 & 0 \\ 0.021 & 0 \\0.022 & 0 \\0 & -0.039 \\ 0 & -0.043 \\ 0 & -0.052 \\ 0 & -0.065
    \end{bmatrix}
\end{align}
Similarly the observer gain matrix $L$ was found to make observer schurr stable and is approximately:
\begin{align}
    L=\begin{bmatrix}
    -0.791	& -0.016 & 0 & 0 & 0 \\
-0.002 & -0.501 & 0 & 0 & -0.022 \\
0 & 0 & -0.272 & -0.025 & 0 \\
0 & 0 & -0.011 & -0.252 & 0 \\
0 & -0.003 & 0 & 0 & -0.240 \\
0 & 0 & -0.013 & -0.258 & 0 \\
0 & 0 & -0.015 & -0.187 & 0 \\
0 & 0 & -0.015 & -0.133	& 0 \\
0 & 0 & -0.014 & -0.091 & 0 \\
0 & -0.004 & 0 & 0 & -0.395 \\
0 & -0.010 & 0 & 0 & -0.145 \\
0 & -0.008 & 0 & 0 & -0.054 \\
0 & -0.005 & 0 & 0 & -0.024 \\
    \end{bmatrix}
\end{align}

The steady state covariance of the residuals, $\Sigma_r$ was approximated by running trajectory following for a straight line down a hallway of approximately 16 meters 40 times. To avoid the effects of the transient behavior at the start of each run, the beggining of each run was ignored. Runs where the localization from google cartographer jumped when updating, were also ignored. The steady state covariance was then approximated by the sample covariance of the remaining data. These experiments were repeated a second time, this time with a watermark being added to the control input. The resulting affect of adding the watermark is shown in figure \ref{fig:traj}. Furthermore each of the detectors was used in post processing on these experimental residuals to approximate the rate of false alarms under various parameters and threshold values. The experimental residuals without watermark were used for all detectors except for Dynamic Watermarking detector which used the second set of experimental residuals. Threshold values for each set of parameters were then found using linear interpolation. Threshold values for the CUSUM at $0.01$ were ignored. These values can be found in table \ref{tab:thresh_exp}.

\begin{table*}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
     \hline
     \multirow{2}{*}{$R_{FA}$} & \multirow{2}{*}{$\chi^2$} & CUSUM & MEWMA & Dyn. Wat. \\
     & & $\gamma=(15~/~17~/~19)$ & $\beta=(0.6~/~0.7~/~0.8)$ &$\ell=(20~/~25~/~30)$ \\\hline
     0.05 & 12.08 & ( 51.04 / 12.27 / 2.21 ) & ( 13.09 / 15.00 / 16.85 ) & ( 99.570 / 103.74 / 105.59 ) \\\hline
     0.03 & 14.29 & ( 655.81 / 384.73 / 158.68 ) & ( 15.05 / 17.59 / 20.17 ) & ( 103.05 / 106.73 / 108.58 ) \\\hline
     0.01 & 21.38 & ( - / - / - ) & ( 20.68 / 24.85 / 28.88 ) & ( 108.582 / 110.79 / 113.94 ) \\\hline
\end{tabular}
    \caption{Experimental thresholds for various parameters}
    \label{tab:thresh_exp}
\end{table*}

\begin{figure}[h]
    \centering
%    \includegraphics{}
    \caption{Effect of watermark on performance}
    \label{fig:traj}
\end{figure}
Two attacks following differing models were then applied. Attack model 1 takes the form:
\begin{align}
    v_n&=-(Cx_n+z_n) +C\xi_n+\zeta_n.\label{eq:attack}
\end{align}
For this style of attack the attack measurement noise $\zeta$ is added to the false state such that $\zeta\sim\mathcal{N}(0,\Sigma_\zeta)$,and the false state $\xi\in\mathbb{R}^p$ is updated according to the closed loop dynamics of the system:
\begin{align}
    \xi_{n+1}&=(A+BK)\xi_n+\omega_n
\end{align}
where the attack process noise $\omega$ is added such that $\omega\sim\mathcal{N}(0,\Sigma_\omega)$. 
The attack process and measurement noise were chosen to leave the distribution of the residuals unchanged. 
Attack model 2 assumes that the attacker adds random noise to the system such that $v_n\sim\mathcal{N}(0,1E-5 I)$.
For each of attack, 10 experimental runs were completed without a watermark and 10 with a watermark for a total of 40 experimental runs.  The beginning of each run, and runs in which cartographer jumps were once again discarded. The runs with a watermark were used in evaluating the dynamic watermarking detector, while all other detectors used the un-watermarked data. The resulting rate of alarm for each of the detection algorithms in the presence of these attacks are displayed in table \ref{tab:exp_exam}.

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|}
     \hline
     Method & $R_{FA}$ & Attack 1 & Attack 2\\\hline
     \multirow{3}{*}{$\chi^2$} & 0.05 & 0.029  &  0.686\\\cline{2-4}
      & 0.03 & 0.012 &  0.622\\\cline{2-4} 
     & 0.01 & 0.000  &  0.467\\\hline
     \multirow{3}{*}{$\underset{\gamma=(15/17/19)}{\text{CUSUM}}$} & 0.05 & ( 0 / 0 / 0 )& ( 0.979 / 0.986 / 0.989 )\\\cline{2-4}
     & 0.03 & ( 0 / 0 / 0 ) & ( 0.812 / 0.856 / 0.921 )\\\cline{2-4} 
     & 0.01 & ( - / - / - ) & ( - / - / - )\\\hline
     \multirow{3}{*}{$\underset{\beta=(0.6/0.7/0.8)}{\text{MEWMA}}$} & 0.05 &( 0.026 / 0.026 / 0.027 ) &( 0.510 / 0.568 / 0.621 )\\\cline{2-4}
     & 0.03 & ( 0.013 / 0.011 / 0.011 ) & ( 0.450 / 0.500 / 0.545 )\\\cline{2-4} 
     & 0.01 & ( 0.001 / 0.001 / 0.000 ) & ( 0.319 / 0.354 / 0.394 )\\\hline
     \multirow{3}{*}{$\underset{\ell=(20/25/30)}{\text{Dyn. Wat.}}$} & 0.05 & ( 0.984 / 0.998 / 1.00 )& ( 1.00 / 1.00 / 1.00 )\\\cline{2-4}
     & 0.03 & ( 0.973 / 0.994 / 0.999 )& ( 1.00 / 1.00 / 1.00 )\\\cline{2-4} 
     & 0.01 & ( 0.949 / 0.983 / 0.996 )& ( 1.00 / 1.00 / 1.00 )\\\hline
\end{tabular}
    \caption{Experimental Results}
    \label{tab:exp_exam}
\end{table}

Note that for the first attack model the rate of alarms appear to drop for the $\chi^2$, CUSUM, and MEWMA detectors. This may be due to the residuals for the un-attacked system not being distributed as a Gaussian distribution resulting in higher threshold values. Since Attack model 1 replaces the feedback completely, the resulting residuals when under attack do follow a Gaussian distribution which then results in lower detection rates. The Dynamic Watermarking detector in the presence of the first attack provides a large increase in the rate of alarms for each set of parameters. For Attack 2 we see that all of the detectors are able to reliably detect the attack.
